Brain Diffusion for Visual Exploration: Cortical Discovery using Large Scale Generative Models

A long standing goal in neuroscience has been to elucidate the functional organization of the brain. Within higher visual cortex, functional accounts have remained relatively coarse, focusing on regions of interest (ROIs) and taking the form of selectivity for broad categories such as faces, places, bodies, food, or words. Because the identification of such ROIs has typically relied on manually assembled stimulus sets consisting of isolated objects in non-ecological contexts, exploring functional organization without robust a priori hypotheses has been challenging. To overcome these limitations, we introduce a data-driven approach in which we synthesize images predicted to activate a given brain region using paired natural images and fMRI recordings, bypassing the need for category-specific stimuli. Our approach -- Brain Diffusion for Visual Exploration ("BrainDiVE") -- builds on recent generative methods by combining large-scale diffusion models with brain-guided image synthesis. Validating our method, we demonstrate the ability to synthesize preferred images with appropriate semantic specificity for well-characterized category-selective ROIs. We then show that BrainDiVE can characterize differences between ROIs selective for the same high-level category. Finally we identify novel functional subdivisions within these ROIs, validated with behavioral data. These results advance our understanding of the fine-grained functional organization of human visual cortex, and provide well-specified constraints for further examination of cortical organization using hypothesis-driven methods.

==> fig_text/S2_S3_FFA.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=1.0\linewidth]{fig_pdf/S2_S3_FFA.pdf}
   \vspace{-5mm}
  \caption{\textbf{Images that excite the fusiform face area.} Voxels in FFA with $t>5$ from the face localizer are used to drive BGDMs. We observe FFA exhibits higher face exclusivity.}
  \vspace{-0.5em}
  \label{fig:FFA}
\end{figure}

==> fig_text/S2_S3_OFA.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=1.0\linewidth]{fig_pdf/S2_S3_OFA.pdf}
   \vspace{-5mm}
  \caption{\textbf{Images that excite the occipital face area.} Voxels in OFA with $t>5$ from the face localizer are used to drive BGDMs. We find subject-wise difference. In \textbf{S2}, OFA is coding for a mixture of faces/text/food. The concept differences are reflected the ground truth NSD and generated BGDM images.}
  \vspace{-0.5em}
  \label{fig:OFA}
\end{figure}

==> fig_text/animate_region_text.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=1.0\linewidth]{fig_pdf/animate_regions.pdf}
   \vspace{-5mm}
  \caption{\textbf{Comparison of S1 person selective regions identified via localizer experiments.}  We identify the $\text{top-}10$ images with highest average activation in the voxels identified via localizer experiments $t>2$. Uncurated except one inappropriate image from fMRI and BGDMs for both categories removed. \textbf{Top:} Images from the two categories used for each localizer experiment. \textbf{Middle:} Images from the ground truth fMRI stimulus set. \textbf{Bottom:} Images generated by BGDMs.}
  \vspace{-0.5em}
  \label{fig:animate}
\end{figure}

==> fig_text/food_region_text.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=1.0\linewidth]{fig_pdf/food_regions.pdf}
   \vspace{-5mm}
  \caption{\textbf{Results for food selective voxels (S1).} \textbf{Top:} Using the food selective voxels identified by \citep{Jain2023}, we visualize the $\text{top-}10$ images with highest average activation from NSD. \textbf{Bottom:} Top images generated by \bdive. We observe that \bdive~  synthesizes food images for these voxels, simply by training using COCO images and brain activations.}
  % \vspace{-0.5em}
  \label{fig:food}
\end{figure}

==> fig_text/inanimate_region_text.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=1.0\linewidth]{fig_pdf/inanimate_regions.pdf}
   \vspace{-5mm}
  \caption{\textbf{Comparison of S1 inanimate category voxels.}  We identify the $\text{top-}10$ images with highest average activation in the voxels identified via localizer experiments $t>2$ without curation. \textbf{Top:} Images from the two categories used for the localizer experiments. \textbf{Middle:} Images from the ground truth fMRI stimulus set. \textbf{Bottom:} Images generated by \bdive.}
  \vspace{-0.5em}
  \label{fig:inanimate}
\end{figure}

==> fig_text/rebut_OFC_text.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=0.95\linewidth]{fig_pdf/rebut_OFC.pdf}
   \vspace{-4mm}
  \caption{\textbf{BrainDiVE applied to orbitofrontal cortex.} We train a voxel-wise encoder for OFC (1029 voxels) in S1 as identified by the HCP mask. NSD images are top-10 out of 10,000 ranked by real response. BrainDiVE top-10 as ranked by our encoder from 100 total generations. The orbitofrontal cortex is not known to respond strongly to visual stimuli, and there does not appear to be a strong semantic trend in the images.}
  \vspace{-0.5cm}
  \label{fig:OFC}
\end{figure}

==> fig_text/rebut_neurogen.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=0.95\linewidth]{fig_pdf/rebut_neurogen.pdf}
   \vspace{-5mm}
  \caption{\textbf{Comparison against NeuroGen.} 
  We visualize the top-10 images for FFA and OFA. Our images exhibit higher visual diversity, and are not restricted to single objects images that dominate ImageNet. NSD images ranked by real response from 10,000 images. In NeuroGen and BrainDiVE, 500 images generated for each region are ranked using the respective encoders for fairness. In FFA, the ground truth images are dominated by human faces. In contrast, NeuroGen generates animal faces, while BrainDiVE shows higher semantic fidelity. In OFA, our work generates diverse images with text and face features, while NeuroGen images show little diversity.}
  \vspace{-0.5cm}
  \label{fig:neurogen}
\end{figure}

==> fig_text/rebut_violin_text.tex <==
\begin{figure}[h!]
  \centering
\includegraphics[width=0.95\linewidth]{fig_pdf/rebut_violin.pdf}
   \vspace{-5mm}
  \caption{\textbf{Predicted activation using an alternative fMRI encoder backbone.} Units are z-scored fMRI BOLD values, higher = more activation. Here we build an fMRI encoder using a frozen \text{EVA02\_CLIP\_B\_psz16\_s8B}, which is different from the \text{CLIP-ViT-B-16-laion2B-s34B-b88K} backbone we use in the paper. We find this new backbone can also achieve high test $R^2$ in the higher visual cortex. For each broad category selective region, we plot the average predicted activation for all NSD images; the top $1\%$ (100 out of 10000) of NSD images ranked by real fMRI activation; and the BrainDiVE images. We find that our images achieve high predicted activation when evaluated with an alternative encoder.}
  \vspace{-0.5cm}
  \label{fig:violin}
\end{figure}
